Permuted AdaIN: Reducing the Bias Towards Global Statistics in Image Classification

Recent work has shown that convolutional neural network classifiers overly rely on texture at the expense of shape cues. We make a similar but different distinction between shape and local image cues, on the one hand, and global image statistics, on the other. Our method, called Permuted Adaptive Instance Normalization (pAdaIN), reduces the representation of global statistics in the hidden layers of image classifiers. pAdaIN samples a random permutation $\pi$ that rearranges the samples in a given batch. Adaptive Instance Normalization (AdaIN) is then applied between the activations of each (non-permuted) sample $i$ and the corresponding activations of the sample $\pi(i)$, thus swapping statistics between the samples of the batch. Since the global image statistics are distorted, this swapping procedure causes the network to rely on cues, such as shape or texture. By choosing the random permutation with probability $p$ and the identity permutation otherwise, one can control the effect's strength. With the correct choice of $p$, fixed apriori for all experiments and selected without considering test data, our method consistently outperforms baselines in multiple settings. In image classification, our method improves on both CIFAR100 and ImageNet using multiple architectures. In the setting of robustness, our method improves on both ImageNet-C and Cifar-100-C for multiple architectures. In the setting of domain adaptation and domain generalization, our method achieves state of the art results on the transfer learning task from GTAV to Cityscapes and on the PACS benchmark.

==> oldtextpieces.tex <==

%The reason that we are amazed by the natural use of camouflage in the animal kingdom is that hiding the shape of a living creature requires a minute attention to details. Only very specific textures can make an animal undetectable. However, in the world of AI, the reliance of current image classifiers on texture makes it such that any change of texture can mislead the classifiers.


% Recent work has shown that convolutional neural network classifiers overly rely on texture at the expense of shape cues. %, which adversely affects the classifier's performance. % in shifted domains.
% % In this work, we make a similar but different distinction between local image cues, including shape and texture, and global image statistics.
% We make a similar but different distinction between shape and local image cues, on the one hand, and global image statistics, on the other.
% Our method, called Permuted Adaptive Instance Normalization (pAdaIN), reduces the representation of global statistics in the hidden layers of image classifiers.
% % We provide a method that enhances the representation of local cues in the hidden layers of image classifiers.
% pAdaIN samples a random permutation $\pi$ that rearranges the samples in a given batch. Adaptive Instance Normalization (AdaIN) is then applied between the activations of each (non-permuted) sample $i$ and the corresponding activations of the sample $\pi(i)$, thus swapping statistics between the samples of the batch. Since the global image statistics are distorted, this swapping procedure causes the network to rely either on global cues such as shape or on local cues. By choosing the random permutation with probability $p$ and the identity permutation otherwise, one can control the strength of this effect. 

% With the correct choice of $p$, fixed apriori for all experiments and selected without considering the test data, our method consistently outperforms baselines in multiple settings. In image classification, our method improves on both CIFAR100 and ImageNet using multiple architectures. In the setting of robustness, our method improves upon the state of the art, both on ImageNet-C and  Cifar-100-C for multiple architectures. In the setting of domain adaptation and domain generalization, our method achieves state of the art results on the translation from GTAV to Cityscapes and on the PACS dataset. 
% % Our method also outperforms baselines as well as in the settings of robustness towards corruptions, domain adaptation and domain generalization. 
% Our code will be made publicly available. 






\subsection{Global texture bias}

% We begin by demonstrating the effect of using pAdaIN on the network's global texture bias. 
% To this end, we first construct a new dataset based on two existing ones: MNIST~\cite{lecun1998gradient}, consisting of handwritten digits representing variable shape, and first 10 classes of KTH surface dataset~\cite{huang2020compact} representing images of soils with variable texture. We use all $10$ classes from each dataset, and resize images from both dataset to $224\times224$ resolution. 
% %and MNIST consists of handwritten digits of resolution $28\times28$ and KTH of soils at resolution $331\times331$. 
% %and resize the  $28\times28$ digit to  $224\times224$ and then randomly crop of a piece of 224x224 out of the texture image to use it. 
% For a given MNIST and KTH image, we blend the images together by inverting the texture according to the digit pixel intensities. We refer to this as TextureMNIST. We create three variants of TextureMNIST: 
% \begin{enumerate}
%     \item Paired TextureMNIST: Every MNIST class (or digit) is assigned a specific KTH class (or texture type). This corresponds to the distribution in natural images whereby every object has a specific texture type. No two digit classes have the same texture class. The number of classes is $10$. The dataset is split to a train, val and test set using the corresponding images int the MNIST and KTH datasets. 
%     \item Random TextureMNIST: Random digits are assigned random textures, from all classes, and in particular, every random digits is assigned many different textures that also exist in other random digits. 
%     %There is no assignment between textures and digits and any digit can be seen with all of the textures.
%     \item Disjoint Random TextureMNIST: As for Random TextureMNIST but with the exception for the assignments in Paired TextureMNIST. That is, there are no images, which use any of the textures or digits from the paired dataset. We use this to evaluate our models' texture and shape bias. In particular we use images from the test set of MNIST and KTH.
% \end{enumerate}

% \begin{figure}
% \centering
% \begin{tabular}{cc}
% Paired TextureMNIST & Random TextureMNIST\\
% \includegraphics[width=0.45\linewidth]{Figures/paired_texture_mnist.png} &
% \includegraphics[width=0.45\linewidth]{Figures/random_texture_mnist.png} \\

% \end{tabular}
% \caption{Examples of TextureMNIST variants. The figure to the left contains distinct texture per digit, while the figure on the right has no assignment between digits and textures. For instance digits 9 and 5 in the bottom row share the same texture background.}
% \label{fig:texturemnistexample}
% \end{figure}

% An illustration of TextureMNIST is given in Fig.~\ref{fig:texturemnistexample}. 
% We train a standard ResNet18 on Paired TextureMNIST dataset. We conducted three evaluations: (1) overall accuracy against the test set of Paired TextureMNIST, (2) texture accuracy, using Disjoint Random TextureMNIST and considering only the label of the texture (3) shape accuracy, again, using Disjoint Random TextureMNIST and considering only the label of the digit. We denote by the shape (resp. texture) bias score, the shape (resp. texture) accuracy normalized by the overall accuracy, denoting the ratio of correct descisions based on shape (resp. texture). 



% % We then evaluate it on Disjoint Random TextureMNIST. That is, given an image in Disjoint Random TextureMNIST, we consider the accuracy of our model with respect to 'texture'  or 'shape' label as assigned for Paired TextureMNIST.     %, where each example has a different texture,digit classes.
% % Our 'texture' accuracy is $95\%$, while the shape accuracy is $1.3\%$. This is inline with observations made by previous works ~\cite{prevwork1, prevwork2}.

% Fig.~\ref{fig:separation}(a) demonstrates the effect for varying values of $p$ as on each of these measures. Fig.~\ref{fig:separation}(b) denotes the shape and texture bias scores. As can be seen, increasing the value of $p$ increases the shape bias, while an intermediate value of $p=0.01$ results in the best overall accuracy. 
% % \sagie{COMPARISON TO INFODROP}

% % Experiment 1: Content vs Texture on TextureMNIST, Resnet18, Variable values of p. 
% % ADD GRAPH HERE (both normalized and unnormalized). 
% % Baselines: BIN, InfoDrop. Run infodrop with different temperature on texturemnist.

% \begin{figure}
% \centering
% \begin{tabular}{cc}
% \includegraphics[width=0.45\linewidth]{Figures/effect_of_p_accuracies.png} &
% \includegraphics[width=0.45\linewidth]{Figures/normalized_accuracies.png} \\
% (a)&(b)\\
% \end{tabular}
% \caption{(a) Analysing the effect of $p$ on the shape accuracy (brown), texture accuracy (green) and overall accuracy (blue) using a Resnet18 architecture, evaluated on TextureMNIST. The $x$-axis denotes the value of $p$ and the $y$-axis, the accuracy. (b) Shape accuracy and texture accuracy of (a) are normalized by the overall accuracy to demonstrate the reliance of the model on shape/texture. }
% \label{fig:separation}
% \end{figure}

% % \sagie{Experiment 2: Evaluation on Imagenet C}
% % \sagie{Experiment 3: CIFAR100 variable p, patch-shuffle + linear classifier}
% % Experiment 2: Fig. 2 of Herman et al. paper (Prevalence of Texture Bias). Add our result for Geiros style transfer, Navon and Imagenet-C datasets. Linear classifier + patch shuffling on cifar100 while varying p.
% % Experiment 3: Comparison to algorithm of Herman et al. paper (Prevalence of Texture Bias) which is basically applying augmentations. Unlike their paper, we improve shape bias *while* increasing overall accuracy. Figure 3 of Texture bias paper. (They show however that for arch, shape is correlated with accuracy). 
% % \sagie{Experiment 4: Visualization:  (a) TSNE on Stylized vs Not Stylized Imagenent on model trained on Imagement with/without PAdaIn.  (b) Explainability methods: SmoothGrad as in InfoDrop Paper. Sagie (c). Accuracy Per Class. (who changed the most vs. vanilla training)}

